SMIRK: 3D Facial Expressions through Analysis-by-Neural-Synthesis

While existing methods for 3D face reconstruction from in-the-wild images excel at recovering the overall face shape, they commonly miss subtle, extreme, asymmetric, or rarely observed expressions. We improve upon these methods with SMIRK (Spatial Modeling for Image-based Reconstruction of Kinesics), which faithfully reconstructs expressive 3D faces from images. We identify two key limitations in existing methods: shortcomings in their self-supervised training formulation, and a lack of expression diversity in the training images. For training, most methods employ differentiable rendering to compare a predicted face mesh with the input image, along with a plethora of additional loss functions. This differentiable rendering loss not only has to provide supervision to optimize for 3D face geometry, camera, albedo, and lighting, which is an ill-posed optimization problem, but the domain gap between rendering and input image further hinders the learning process. Instead, SMIRK replaces the differentiable rendering with a neural rendering module that, given the rendered predicted mesh geometry, and sparsely sampled pixels of the input image, generates a face image. As the neural rendering gets color information from sampled image pixels, supervising with neural rendering-based reconstruction loss can focus solely on the geometry. Further, it enables us to generate images of the input identity with varying expressions while training. These are then utilized as input to the reconstruction model and used as supervision with ground truth geometry. This effectively augments the training data and enhances the generalization for diverse expressions. Our qualitative, quantitative and particularly our perceptual evaluations demonstrate that SMIRK achieves the new state-of-the art performance on accurate expression reconstruction. Project webpage: https://georgeretsi.github.io/smirk/.

==> sections_camera_ready/04_method_before_radekal_compression.tex <==
\section{Methodology}

\subsection{Overview}
\label{sec:overview}

%The core concept can be summarized as \emph{enhancing 3D face reconstruction through visual guidance}.

%\textcolor{red}{rephrase it}
The proposed pipeline relies on a image reconstruction rationale: we start from a face image, we use an encoder to estimate the parameters of a 3D morphable model (FLAME~\cite{li2017flame} - more information can be found in the Suppl. Mat.), render an image of the predicted face \textbf{geometry}, and then we use an image-to-image generator to reconstruct the initial image. 
Under such a framework, learning can be performed by directly comparing the initial and the reconstructed image. 
This is in contrast to previous approaches on 3D face reconstruction\cite{danecek2022emoca,feng2021learning,deng2019accurate} which render a textured face (which also requires predicting albedo and lighting) in order to accommodate their self-supervision scheme.
Notably, this means that neural-network based losses such as perceptual~\cite{johnson2016perceptual}, identity\cite{zielonka2022mica,deng2019accurate} or emotion~\cite{danecek2022emoca} can be used to compare the reconstructed and input images without the domain-gap problem which may introduce artifacts. \todo{say something about l1 or not ? it helps that too}

% our approach directly attempts to reconstruct the initial image. Notably, our approach also does not suffer from the domain gap problem between the input and the rendered image and thus perceptual neural-network based losses such as identity\cite{zielonka2022mica} or emotion\cite{danecek2022emoca} which can lead to artifacts when the gap exists, here they do not.
% \textcolor{red}{Contrary to APPROACHES, we do not heavily rely on extra losses that may lead to artifacts. ++}


Of course, reconstructing an image from a 3D FLAME face without any extra ``help" is more related to the neural rendering field. We stress that we do not try to perfectly reconstruct the input image.  \textcolor{red}{Contrary to APPROACHES, we do not strive for a realistic rendering approach for image reconstruction. ++}

Nonetheless, in this work, we rely on a guided inpainting approach, where parts of the initial image are given as prior for the image reconstruction and the guidance comes from the \textcolor{red}{non-texture rendering} of the 3D face mesh.  
The key idea here is to mask out the actual face of the person from the initial in-the-wild image. 
Then implicitly impose the system to actually rely on the rendered mesh to recreate the initial image. 
This way, the ``non-interesting" background is given as input for the reconstruction step and thus the model can focus on the facial features. 

Architecture-wise, we consider two core models to be trained:
\begin{itemize}
    \item \textbf{Encoder:} estimates the FLAME representation from a face image. %should be lightweight.
    \item \textbf{Image-to-Image Translator:} takes as input the concatenation of the masked-out input image, where the face is ``hidden", and the rendered mesh of the predicted 3D reconstruction and outputs a new image.  %should promote gradient flow. 
\end{itemize}
Auxiliary models are used as non-trainable off-the-self modules for calculating perceptual-oriented losses, such as identity or emotion loss. 

To unlock the capabilities of the proposed pipeline, we distinguish two paths:
\begin{enumerate}
    \item \textbf{Image Reconstruction Path:} A face image is given as input and subsequently reconstructed with our translator, comprising the visual supervision step. The overview of this path is given in Figure~\ref{fig:reconstruction}.
    \item \textbf{Cycle Path:} An augmented expression representation is given as an input, used for reconstructing a realistic face through the generator and then subsequently projected to the expression space again through the encoder. This path aims to impose consistency, loosely based to the Cycle-GAN~\cite{zhu2017cyclegan} approach, and promotes generalization by generating unseen reconstructed faces.
    Its overview can be found in Figure~\ref{fig:cycle}.
\end{enumerate}

The aforementioned framework manages to provide accurate 3D reconstruction without the need for perceptual losses.
Nonetheless, perceptual losses can be extremely useful as have been seen before (e.g., emotions in \cite{danecek2022emoca}, lip reading in \cite{filntisis2023spectre}).
To this end, we can optionally include such perceptual losses in the proposed pipeline. 
Under the proposed framework, these losses would be applied on the reconstructed images, practically minimizing the domain gap that appeared in previous approaches \textcolor{red}{(e.g. \cite{filntisis2023spectre} ...)}

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/overview_reconstruction-cropped (1).pdf}
    \caption{
    \textbf{Reconstruction pass.} An input image is passed into the encoder which regresses FLAME and camera parameters. 
    A 3D shape is reconstructed, rendered with a differentiable renderer and finally translated into the output domain with the image translation network. 
    Then, standard self-supervised landmark, photometric and perceptual losses are computed.
    }
    \label{fig:reconstruction}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/overview_cycle-cropped (1).pdf}
    \caption{
    \textbf{Augmented cycle pass.} 
    The FLAME expression parameters of an existing reconstruction are modified. The resulting modified face is then rendered using our neural renderer. 
    The rendering is then passed to the face reconstruction encoder to regress the FLAME parameters and a consistency loss between the modified input and reconstructed FLAME parameters is computed. 
    }
    \label{fig:cycle}
\end{figure}

\subsection{Learn via Analysis by Image Synthesis}

%In this section, we focus on the main novelty of our work, namely training through the translator reconstruction. 
% The are two major pipelines to be described, namely reconstruction path and the cycle path, both crucial for our method's performance.
\modelName is supervised with to different passes, the reconstruction path and the augmented-cycle path.
%; thus dubbing our method \emph{\modelName}. 
In this section, we will describe in detail the components of these paths and how these paths are optimized with respect to our encoder and translator models.


\subsubsection{Description of the Models}

\qheading{Face Model:}
In this work, we rely on the FLAME model \cite{li2017flame} to express the 3D geometry of a face. In particular, FLAME generates a mesh comprising $\numverts=5023$ vertices, which can be deformed according to a set of intuitive parameters:  
rigid head pose $\boldsymbol{\theta_{p}}$, orthographic camera parameters~$\boldsymbol{c}$, identity parameters $\boldsymbol{\beta}$, expression parameters $\boldsymbol{\psi}$ (extended with parameters which model \emph{eye close}~\cite{zielonka2022mica}), and pose adjustments specifically for the jaw $\boldsymbol{\theta}_{jaw}$ parameters. 
% Unlike the original FLAME model, our model's expression basis contains additional two vectors for eye closure, one for each eyelid.

In this work, we split the aforementioned parameters that need to be predicted into three subsets:
\begin{itemize}
    \item \emph{head pose} set $\boldsymbol{\theta'}$, that contains both the rigid head pose $\boldsymbol{\theta_{p}}$ and the orthographic camera parameters~$\boldsymbol{c}$, forming a global representation of the head spatial placement. 
    \item \emph{identity} set $\boldsymbol{\beta}'$, that only contains the typical identity shape parameters.
    \item \emph{expression} set $\boldsymbol{\psi}'$, that contains the expression parameters $\boldsymbol{\psi}$ (extended with eyelid closure) along with jaw parameters $\boldsymbol{\theta}_{jaw}$. This set is responsible of controlling any possible facial expression. 
\end{itemize}
% \textcolor{red}{check this subsets - not to be confused with typical definitions in FLAME!}

%\\

%Next, $S$ is concatenated along with a masked version $M(I)$ of the original input image, and the combined result is fed into an image-to-image generator which tries to reconstruct the original input image I (denoted as $I'$).

%As it seems the overall concept of our method is simple: in order to minimize the reconstruction loss between the reconstructed image $I'$ and the input image $I$, the image encoder $E$ is forced to capture facial shape and expression details, so that these can then be used to successfully guide the generator $D$ in his reconstruction.
 


%Having described the functionality of the two core models, let us delve into the critical architectural details. 
%One common denominator for both models is the simplicity 

%\break
\qheading{Encoder:}
Starting from an input image $I$, an encoder $E$ is used to predict the parameters of the aforementioned FLAME 3D morphable model.
%As stated before, \emph{Encoder} estimates a set of FLAME parameters. 
%In this work, we focus only on the expression part, training a network to jointly predict the 50 expression parameters, the 3 jaw pose parameters and the 2 eyelid parameters in order to fully control the facial expressions. 
In this work, we focus only on the expression part, using a network to predict the augmented \emph{expression} set $\boldsymbol{\psi}'$ ($50$ parameters for expression, $3$ for jaw pose and $2$ for the eyelids). 
Different networks are used for pose estimation and identity shaping so as to not interfere with the main expression model. 
Overall, we used three distinct MobileNetv3~\cite{howard2019searching} models to predict the complete set of the FLAME parameters, aiming to a \emph{lightweight} backbone.
The encoder is then a set of three submodels: $E = \{ E_{\boldsymbol{\theta'}},  E_{\boldsymbol{\beta'}},  E_{\boldsymbol{\psi'}} \}$
Following the aforementioned annotation, we have: 
\begin{equation}
  \boldsymbol{\theta'} = E_{\boldsymbol{\theta'}}(I), \quad 
  \boldsymbol{\beta'} = E_{\boldsymbol{\beta'}}(I), \quad 
  \boldsymbol{\psi'} = E_{\boldsymbol{\psi'}}(I)
\end{equation}
%\\


%\break
\qheading{Image-to-Image Translator:}
Given a rendered mesh of the 3D face $S$ and the masked-out input image $M(I)$, the \emph{Image-to-Image Translator} tries to reconstruct the initial image $I$. 
The two input images, $S$ and $M(I)$ are concatenated and are given as input to the Translator $T$, so the process is formulated as:
\begin{equation}
    I' = T(S \oplus M(I))
\end{equation}
where $M(.)$ is a masking function and $\oplus$ denotes concatenation.
This process is essentially an image-to-image translation (even though the initial ``image" is a concatenation of two images) and thus a UNet architecture~\cite{RonnebergerFB15unet} is adopted. 
Its functionality relies on the usage of the estimated 3D geometry to reconstruct the initial faces characteristics.  
 
A crucial property of this module is to assist the gradient flow towards the encoder. 
%This way, both the reconstruction path and the cycle path will be more easily trained and ``collapsing" of solutions (e.g., generating non-realistic reconstructions) can be avoided. 
Therefore, a UNet-based architecture is ideal, since the existing shortcuts allow the gradient to flow uninterrupted. 



\subsubsection{Reconstruction Path}

The reconstruction path, as outlined in Figure~\ref{fig:reconstruction}, is the core pipeline for the proposed visual reconstruction scheme.
The process is straightforward: project the input image into the FLAME parameter space through the Encoder and use the rendered 3D face image along with a masked image to reconstruct the input image through the Image-to-Image Translator, formulated as:
\begin{equation}
I' = T(R(E_{\boldsymbol{\theta'}}(I), E_{\boldsymbol{\beta'}}(I), E_{\boldsymbol{\psi'}}(I)) \oplus M(I))
\end{equation}
In the proposed pipeline we focus on optimizing the \emph{expression encoder} $E_{\boldsymbol{\psi'}}$, while the other encoder are kept fixed.


\qheading{Rendering:}
Using the parameters predicted by the encoder we first differentiably render an image $S$ of the \textbf{geometry} of the 3D model. Note that although the full FLAME mesh includes also ears, eyeballs, neck, and scalp in the facial mesh, in our work we only render the \textit{expressive} part of the 3D model, which is the face. Images of this rendering can be seen in the pipeline figures (e.g. Fig.~\ref{fig:reconstruction}).

% \begin{equation}
%   S = R(\boldsymbol{\theta'}, \boldsymbol{\beta}', \boldsymbol{\psi}')  
% \end{equation}

% The used renderer $R$ takes into accout a part of FLAME rendering. mouth and eyes are ``empty".


\qheading{Impact of Masking:}
The masking function $M(I)$  of the initial image $I$ is a very crucial step towards reliable generation of the reconstructed images.
To promote the reliance from the 3D rendered face, we need to ``remove" the face of the input image. 
Specifically, we use the convex hull of detected 2D landmarks~\cite{bulat2017far} and dilate it in order to completely cover the input face.
The precision of the landmarks' position is not critical, since this masking out step aims to simply remove the inner structure of the face.
Without any information of face interior, training the translator becomes challenging. For example, texture information, such as skin color, facial hair or even accessories (e.g., glasses) are ``distractors" that complicate training. 
One way to address this issue, is to keep a small number of pixels from the interior of the face mask. 
Specifically, we retain a very small amount ($0.5\%$) of pixels, randomly selected, to be used as a guidance for reconstruction.
Note that if we use a larger number of pixels, the reconstruction becomes too guided and the 3D rendered face does not control the reconstruction output adequately. 
The same behavior was met when we tried to randomly mask out blocks of the image, as done in ~\cite{he2022autolink}.
%and the cycle path cannot faithfully reconstruct new expressions. 

A final addition to the masking process is done by extracting a mask of the rendered 3D face and allowing random pixels only from the face interior that lie into this mask. 
The idea behind this extra step is to also mask-out pixels from inside the mouth and thus penalize ``heavy" inpainting actions, such as extending the lips because a pixel that correspond to lip was found inside the predicted mouth region. 
An example of such an error can be seen in Figure~\ref{fig:masking_error}.
%This is very helpful for the cycle path also. 

\iffalse
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/masking-procedure-cropped.pdf}
    \caption{+++.}
    \label{fig:masking_procedure}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/masking_error-cropped.pdf}
    \caption{Impact of rendered face mask on the overall masking scheme. If points are used from within the mouth, the system can learn an inpainting solution that resembles a closed mouth, even if this is not the case.}
    \label{fig:masking_error}
\end{figure}
\fi

\begin{figure}
    \centering
    \begin{tabular}{cc}
     \includegraphics[width=.76\linewidth]{figures/masking-procedure-cropped (1).pdf}    & 
     \includegraphics[width=.18\linewidth]{figures/masking_error-cropped (1).pdf}\\
      (a)   & (b) 
    \end{tabular}
    \caption{\textbf{Neural rendering module.} 
    (a) \emph{Masking process.} An input image is masked to obscure the face (left), then we sample random pixels to be unmasked (right).
    (b) \emph{Image translation.} An input image (top) is concatenated with differentiable rendering of the input mesh (middle) and passed through the neural renderer to produce the output image(bottom).
    }
    \label{fig:masking_procedure}
\end{figure}

\qheading{Considered Losses:}
Optimization of such a reconstruction scheme, can be formulated through a loss that directly compares the reconstructed image with the initial one. To further enhance the performance of the proposed framework a set of losses is considered, as described below.
\begin{itemize}
    \item \emph{Image Reconstruction Losses:}
    %reconstruction loss: perceptual \& L1
%both losses required for the best possible results. (VGG-based) perceptual loss helps the fast convergence of a meaningful structure of the face, while L1 helps with appearance finer details.
    Reconstruction is optimized through two complementary losses. Specifically, we minimize the difference of the original image and the reconstructed image by 1) the perceptual loss of \cite{johnson2016perceptual} that uses multi-scale features and promotes structure similarity, as done in Autolink~\cite{he2022autolink}, and 2) $L_1$ loss. This can be written as:
    \begin{equation}
        \mathcal{L}_{rec} = \frac{1}{N}\sum_{i=1}^{N} \big( \|\Gamma({I'}_i) - \Gamma(I_i)\|_2^2 +  \| {I'}_i - I_i\|_1 \big)
    \end{equation}
    where $\Gamma()$ represents the perceptual encoder of \cite{johnson2016perceptual}.
    This VGG-based perceptual loss helps the fast convergence of a meaningful structure of the face, while the $L_1$ loss helps with the appearance of finer details.
    \item \emph{Landmark Loss:}
    Typical landmark loss is considered between detected landmarks of the input image and the corresponding landmarks, extracted from the 3D FLAME model. \textcolor{red}{@filby - more details}. \textcolor{red}{This loss acts as a guidance and has been proven not crucial for the proposed framework - remove it if no ablation is given}.
    \item \emph{Regularization:}
    We also use $L_2$ regularization over the expression parameters. This is complementary to the landmark loss in the sense of acting as a constraint to avoid extreme, non-realistic, expressions. 
    \item \emph{Task-Specific Perceptual Losses:}
    Finally, one can consider task-specific perceptual losses, that model adequately well subspaces of the actual expression space. 
    Specifically, we consider an \emph{emotion loss}, as done in EMOCA~\cite{danecek2022emoca}, that relies on a pre-trained network trained specifically for the respective task. In our case, we use the same pretrained network with EMOCA\cite{danecek2022emoca}, which is a Resnet50 model trained on AffectNet\cite{mollahosseini2017affectnet}.
    Given the emotion prediction network $P_e$, the loss is formulated as the reconstruction perceptual loss:
    \begin{equation}
    \mathcal{L}_{perc} = \frac{1}{N}\sum_{i=1}^{N} \| P_e({I'}_i) - P_e(I_i)\|_2^2 
    \end{equation}
    In more detail, we ``freeze" the translator $T$ for this step, and optimize only the Encoder $E_{\boldsymbol{\psi'}}$, since we do not want the loss to affect the translator. 
    The benefit of using such perceptual losses over the proposed framework is that the domain gap problem is minimized, since the two compared images are in the same space (e.g., EMOCA used a texture-rendered image for comparison).
    
    %Specifically, two such losses were considered: \emph{emotion loss}, as done in EMOCA~\cite{danecek2022emoca} and \emph{lip-read loss}, as done in SPECTRE~\cite{filntisis2023spectre}. Both losses employ pre-trained networks, trained specifically for the respective tasks, and used ``frozen" to back-propagate perceptual information to our models. In more detail, we also ``freeze" the Image-to-Image Translator for this step, and optimize only the Encoder, since we do not want these losses to affect the Image-to-Image Translator. 
    %It should be noted that these losses lead to over-exaggeration of some expressions if not regularized properly; the simplest way to do this is by using the landmark loss with a non-trivial weight.
    %The benefit of using such perceptual losses over the proposed framework is that the domain gap problem is minimized, since the two compared images are in the same space (e.g., EMOCA/SPECTRE used a texture-rendered image for comparison). 
    
\end{itemize}

%\textbf{Training of the Encoder:}


\subsubsection{Cycle Path}

%It's not only about consistency - it promotes (quite aggressively) variations

The aforementioned reconstruction concept could be a powerful tool but is limited from the encoder learning process. 
For example, if a more complex lip structure, scarcely seen in the training data, cannot be reproduced quickly enough from the encoder, the translator could learn to correlate miss-aligned lip structure and thus multiple similar, but distinct, facial expressions will be \emph{collapsed} to a single reconstructed representation. 

This issue can be addressed with a \emph{cycle consistency} path, where different expression parameters $\boldsymbol{\psi'}$ should be successfully retrieved through the image reconstruction process. 
The basic concept is straightforward: start from the FLAME parameter space, reconstruct a realistic image with the Image-to-Image Translator and then re-estimate the expression parameters using the Encoder. 
%We start from a set of FLAME parameters, we render the corresponding mesh and then we reconstruct a realistic face.  
Then a cycle consistency loss is directly used on the parameter space, enforcing the predicted expression parameters to be as close as possible to the initial ones.  
This concept is visualized in Figure~\ref{fig:cycle}.

%\textcolor{red}{refer to works with similar motivation and cycle losses}

\qheading{Promoting Diverse Expressions:}
Despite its value, such a consistency loss alone is not enough to distinguish between the many possible facial expressions. 
If any of these paths, reconstruction or cycle, does not contains meshes with ``complex" structure, the aforementioned expression collapse to a reduced set of reconstructed face images is unavoidable. To this end, this cycle path does not only enforce cycle consistency, but most importantly \emph{promotes variations in the expression parameter space}.    
This way, we let the system ``see" expression parameters that typically are not that common.

To effectively augment the cycle path with interesting variations, the following steps are considered:
\begin{itemize}
%\item extend the batch be repeating K times
\item \textbf{Permutation:} permute the expressions in a batch. Note that permuting expressions within a batch is a simple yet effective solution. However, to unlock the potential of such a solution, at least a subset of the training dataset should contain ``intense" expressions (e.g., emotion).
\item \textbf{Perturbation:} add non-trivial noise to the expression parameters.
\item \textbf{Template Injection:} use expression templates of ``difficult" / scarce expressions. To obtain these expression parameters for FLAME we perform direct iterative parameter fitting on the FaMoS~\cite{bolkart2023instant} dataset which depicts multiple subjects perform extreme and assymetric expressions.
\item \textbf{Zero Expression:} once in a while, one should consider neutral expressions to not bias the system towards complex only cases. 
\end{itemize}
For all the possible expression augmentations, we simultaneously simulate jaw and eyelid openings/closings. These jaw and eyelid augmentations are more ``aggressive" in the zero-expression case, since specific intense expressions may not blend together well with further augmentations.
Visual examples of all the presented categories of expression augmentations can be seen in Figure~\ref{fig:cycle_expressions}, along with the ability of the UNet to generate close to realistic images, simulating emotions etc. in the initial image domain. 
\\

\begin{figure*}
    \centering
    \includegraphics[width=.95\linewidth]{figures/cycle_expressions-cropped.pdf}
    \caption{
    \textbf{Neural expression augmentation.} 
    \textcolor{red}{to be updated with new images} 
    Our neural renderer enables us to modify the expression, generating a new training image-3D face training pair. 
    We can edit the expression with random noise, permutation from other reconstructions, 
    \textcolor{red}{template injection?}
    \textcolor{red}{The zero expression with eyes closed is confusing }
    }
    
    \label{fig:cycle_expressions}
\end{figure*}


%\textcolor{red}{add images to highlight augmentation}



%\textcolor{red}{Note that permuting expressions within a batch is a simple yet effective solution. However, to unlock the potential of such a solution, at least a subset of the training dataset should contain ``intense" expressions (e.g., emotion). Then the permutation step will transfer this expressions to the whole training set.} 


\qheading{Considered Losses:}
The consistency loss is the mean-squared error between the given augmented expression parameters $\psi_{a}$ and the predicted expressions at the end of the cycle path:
\begin{equation}
    \mathcal{L}_{cycle} = \frac{1}{N}\sum_{i=1}^{N} \|
     E_{\boldsymbol{\psi'}}(T(R(E_{\boldsymbol{\theta'}}(I), E_{\boldsymbol{\beta'}}(I), \psi_{a})
     - \psi_{a}\|_2^2 
\end{equation}
The optimization is performed on both the Encoder and the Image-to-Image Translator, opting to fine-tune their functionality and impose consistency. 
Essentially, a one-to-one correspondence is desired between the 3D FLAME face and the reconstructed image. 

A potential problem with this extra cycle path is that the Image-to-Image Translator can be ``over-fitted" in order to create a non-realistic, render-like plain reconstruction (see Suppl. Material), since no supervision is in place to retain realistic images in this path. 
We have seen that with appropriate weight on the aforementioned cycle loss, we can avoid this problem, but the sensitivity remains.
This issue can be addressed by introducing an additional identity loss, that constraints the generated image to correspond to the same person as the initial input image. 
As the identity loss, the \textcolor{red}{@filby} is used, akin to previous perceptual losses. 

%\qheading{Face Image Manipulation}

%A by-product of the proposed methodology is the creation of a well-performing face manipulation system, despite the simplicity of the translator.

\iffalse
%\subsection{Loss Formulation}

%reconstruction loss: perceptual \& L1
%both losses required for the best possible results. (VGG-based) perceptual loss helps the fast convergence of a meaningful structure of the face, while L1 helps with appearance finer details.

%cycle loss (MSE)

%(NOT NEEDED) landmark loss as guidance (minor impact)

\subsubsection{Extra perceptual losses}

Extra considered losses for ablation:
emotion, lip read.

Note that the considered domain is the reconstructed images, thus no domain gap exists. 

\fi


%\subsubsection{Face Image Manipulation}

%A by-product of the proposed methodology is the creation of a well-performing face manipulation system, despite the simplicity of the generator.

\subsubsection{Implementation Details?}
\textcolor{red}{@filby "random" implementation details??}

\textcolor{red}{Note that the non-textured rendered mesh is used as input. Preliminary experimentation showed no difference in performance when the texture from DECA was added.}   

\textcolor{red}{check this}
The Image-to-Image Translator can be seen as a neural renderer alternative. 
However, contrary to such approaches, we do not aim to have a realistic rendering per-se, but rather have a lightweight and elegant guided \emph{inpainting} approach that heavily relies on the 3D geometry. 
This will be further highlighted by the masking step. 

\todo{pretrain details?}
A shape regularizer is also in place to impose identity shaping with respect to a pre-trained network, such as DECA~\cite{feng2021learning} or MICA~\cite{zielonka2022mica}. 







==> sections_camera_ready/4_methodology_old.tex <==
\section{Methodology}

\iffalse
\subsection{Preliminaries}
\label{sec:prelims}
\qheading{Face Model:}
The FLAME model \cite{li2017flame}, is a comprehensive statistical 3D head model. 
It incorporates parameters for identity shaping $\shapecoeff \in \mathbb{R}^\shapedim$, facial expressions $\expcoeff \in \mathbb{R}^\expdim$, and pose adjustments $\posecoeff \in \mathbb{R}^{3\numjoints+3}$, accommodating rotations around $\numjoints = 4$ pivotal joints—these include the neck, jaw, and both eyeballs—as well as the overall head rotation.
Unlike the original FLAME model, our model's expression basis contains additional two vectors for eye closure, one for each eyelid.
Given these parameters, FLAME generates a mesh comprising $\numverts=5023$ vertices.
In a formal representation, FLAME can be expressed as:
\begin{equation}
% (\mathbf{V}, \mathbf{F}) = \flamev(\shapecoeff, \posecoeff, \expcoeff),
\flamev(\shapecoeff, \posecoeff, \expcoeff)\rightarrow (\mathbf{V}, \mathbf{F}),
\end{equation}
where the model's vertices are denoted as $\mathbf{V} \in \mathbb{R}^{\numverts \times 3}$ and it includes $\numfaces = 9976$ facial components $\mathbf{F} \in \mathbb{R}^{\numfaces \times 3}$.
\fi

\subsection{Overview}
\label{sec:overview}

The core concept can be summarized as \emph{enhancing 3D face reconstruction through visual guidance}.
%, aiming to ``discover" finer details.
%\textcolor{red}{rephrase it}
The proposed pipeline relies on a image reconstruction rationale: we start from a face image, we use an encoder to estimate the parameters of a 3D morphable model (FLAME\cite{li2017flame} - more information can be found in the Suppl. Mat.), render an image of the predicted face \textbf{geometry}, and then we use an image-to-image generator to reconstruct the initial image. 
Under such a framework, learning can be performed by directly comparing the initial and the reconstructed image. This is in contrast to previous approaches on 3D face reconstruction\cite{danecek2022emoca,feng2021learning,deng2019accurate} which render a textured face (which also requires predicting albedo and lighting) in order to accommodate their self-supervision scheme.
Notably, this means that neural-network based losses such as perceptual~\cite{vgg}, identity\cite{zielonka2022mica,deng2019accurate} or emotion~\cite{danecek2022emoca} can be used to compare the reconstructed and input images without the domain-gap problem which may introduce artifacts. \todo{say something about l1 or not ? it helps that too}

% our approach directly attempts to reconstruct the initial image. Notably, our approach also does not suffer from the domain gap problem between the input and the rendered image and thus perceptual neural-network based losses such as identity\cite{zielonka2022mica} or emotion\cite{danecek2022emoca} which can lead to artifacts when the gap exists, here they do not.
% \textcolor{red}{Contrary to APPROACHES, we do not heavily rely on extra losses that may lead to artifacts. ++}


Of course, reconstructing an image from a 3D FLAME face without any extra ``help" is more related to the neural rendering field. We stress that we do not try to perfectly reconstruct the input image.  \textcolor{red}{Contrary to APPROACHES, we do not strive for a realistic rendering approach for image reconstruction. ++}

Nonetheless, in this work, we rely on a guided inpainting approach, where parts of the initial image are given as prior for the image reconstruction and the guidance comes from the \textcolor{red}{non-texture rendering} of the 3D face mesh.  
The key idea here is to mask out the actual face of the person from the initial in-the-wild image. 
Then implicitly impose the system to actually rely on the rendered mesh to recreate the initial image. 
This way, the ``non-interesting" background is given as input for the reconstruction step and thus the model can focus on the facial features. 

Architecture-wise, we consider two core models to be trained:
\begin{itemize}
    \item \textbf{Encoder:} estimates the FLAME representation from a face image. %should be lightweight.
    \item \textbf{Image-to-Image Translator:} takes as input the concatenation of the masked-out input image, where the face is ``hidden", and the rendered mesh of the predicted 3D reconstruction and outputs a new image.  %should promote gradient flow. 
\end{itemize}
Auxiliary models are used as non-trainable off-the-self modules for calculating perceptual-oriented losses, such as identity or emotion loss. 

To unlock the capabilities of the proposed pipeline, we distinguish two paths:
\begin{enumerate}
    \item \textbf{Image Reconstruction Path:} A face image is given as input and subsequently reconstructed with our translator, comprising the visual supervision step. The overview of this path is given in Figure~\ref{fig:reconstruction}.
    \item \textbf{Cycle Path:} An augmented expression representation is given as an input, used for reconstructing a realistic face through the generator and then subsequently projected to the expression space again through the encoder. This path aims to impose consistency, loosely based to the Cycle-GAN~\cite{} approach, and promotes generalization by generating unseen reconstructed faces.
    Its overview can be found in Figure~\ref{fig:cycle}.
\end{enumerate}

The aforementioned framework manages to provide accurate 3D reconstruction without the need for perceptual losses.
Nonetheless, perceptual losses can be extremely useful as have been seen before (e.g., emotions in \cite{danecek2022emoca}, lip reading in \cite{filntisis2023spectre}).
To this end, we can optionally include such perceptual losses in the proposed pipeline. 
Under the proposed framework, these losses would be applied on the reconstructed images, practically minimizing the domain gap that appeared in previous approaches \textcolor{red}{(e.g. \cite{filntisis2023spectre} ...)}

\begin{figure*}
    \centering
    \includegraphics[width=.6\linewidth]{figures/overview_reconstruction-cropped.pdf}
    \caption{reconstruction overview}
    \label{fig:reconstruction}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=.6\linewidth]{figures/overview_cycle-cropped.pdf}
    \caption{cycle overview}
    \label{fig:cycle}
\end{figure*}

%FIGURE!
\iffalse
\subsection{Models Description}

\qheading{Face Model:}
In this work, we rely on the FLAME model \cite{li2017flame} to express the 3D geometry of a face. In particular, FLAME generates a mesh comprising $\numverts=5023$ vertices, which can be deformed according to a set of intuitive parameters:  
rigid head pose $\boldsymbol{\theta_{p}}$, orthographic camera parameters~$\boldsymbol{c}$, identity parameters $\boldsymbol{\beta}$, expression parameters $\boldsymbol{\psi}$ (extended with parameters which model eye close~\cite{zielonka2022mica}), and pose adjustments specifically for the jaw $\boldsymbol{\theta}_{jaw}$ parameters. 
We split the parameters that need to be predicted into three subsets:
\begin{itemize}
    \item \emph{head pose} set $\boldsymbol{\theta_{p}^{'}}$, that contains both the rigid head pose $\boldsymbol{\theta_{p}}$ and the orthographic camera parameters~$\boldsymbol{c}$, forming a global representation of the head spatial placement. 
    \item \emph{identity} set $\boldsymbol{\beta}^{'}$, that only contains the typical identity shape parameters.
    \item \emph{expression} set $\boldsymbol{\psi}^{'}$, that contains the expression parameters $\boldsymbol{\psi}$ (extended with eyelid closure) along with jaw parameters $\boldsymbol{\theta}_{jaw}$. This set is responsible of controlling any possible facial expression. 
\end{itemize}
% \textcolor{red}{check this subsets - not to be confused with typical definitions in FLAME!}
After prediction, these parameters are used to differentiably render an image of the \textbf{geometry} of the 3DMM, denoted as $S$. Next, $S$ is concatenated along with a masked version $M(I)$ of the original input image, and the combined result is fed into an image-to-image generator which tries to reconstruct the original input image I (denoted as $I^{'}$).

%As it seems the overall concept of our method is simple: in order to minimize the reconstruction loss between the reconstructed image $I^{'}$ and the input image $I$, the image encoder $E$ is forced to capture facial shape and expression details, so that these can then be used to successfully guide the generator $D$ in his reconstruction.
 


%Having described the functionality of the two core models, let us delve into the critical architectural details. 
%One common denominator for both models is the simplicity 

\qheading{Encoder}

Starting from an input image $I$, an encoder $E$ is used to predict the parameters of the FLAME 3D morphable model:

As stated before, \emph{Encoder} estimates a set of FLAME parameters. In this work, we focus only on the expression part, training a network to jointly predict the 50 expression parameters, the 3 jaw pose parameters and the 2 eyelid parameters in order to fully control the facial expressions. 
Different networks are used for pose estimation and identity shaping so as to not interfere with the main expression predictor model. 
Overall, we used three distinct models to predict different sets of the FLAME parameters.
For all three models, we used MobileNetv3 architectures~\cite{}, aiming towards a lightweight backbone. 

\qheading{Image-to-Image Translator}

Given a rendered mesh of the 3D face and the masked-out input image, the \emph{Image-to-Image Translator} tries to reconstruct the initial image. This process is essentially an image-to-image translation (even though the initial ``image" is a concatenation of two images) and thus a UNet architecture~\cite{} is adopted. Its functionality relies on the usage of the estimated 3D geometry to reconstruct the initial faces characteristics.  
\textcolor{red}{Note that the non-textured rendered mesh is used as input. Preliminary experimentation showed no difference in performance when the texture from DECA was added.}    

A crucial property of this module is to assist the gradient flow towards the encoder. 
This way, both the reconstruction path and the cycle path will be more easily trained and ``collapsing" of solutions (e.g., generating non-realistic reconstructions) can be avoided. 
Therefore, a UNet-based architecture is ideal for this module, since the existing shortcut connection allow the gradient to flow uninterrupted. 

\textcolor{red}{check this}
The Image-to-Image Translator can be seen as a neural renderer alternative. 
However, contrary to such approaches, we do not aim to have a realistic rendering per-se, but rather have a lightweight and elegant guided \emph{inpainting} approach that heavily relies on the 3D geometry. 
This will be further highlighted by the masking step. 

%focus on generator and gradient flow

%UNet as a simple, gradient-assisting, architecture.
\fi

\subsection{Learn via Analysis by Image Synthesis}

%In this section, we focus on the main novelty of our work, namely training through the translator reconstruction. 
The are two major pipelines to be described, namely reconstruction path and the cycle path, both crucial for our method's performance; thus dubbing our method \emph{RecCycle}. 
In this section, we will describe in detail the components of these paths and how these paths are optimized with respect to our encoder and translator models.


\subsubsection{Description of the Models}


\qheading{Face Model:}

Starting from an input image $I$, an encoder $E$ is used to predict the parameters of the FLAME 3D morphable model: rigid head pose $\boldsymbol{\theta_{p}}$, orthographic camera parameters~$\boldsymbol{c}$, identity parameters $\boldsymbol{\beta}$, expression parameters $\boldsymbol{\psi}$ (extended with parameters which model eye close\cite{zielonka2022mica}), and pose adjustments specifically for the jaw $\boldsymbol{\theta}_{jaw}$ parameters. 

Unlike the original FLAME model, our model's expression basis contains additional two vectors for eye closure, one for each eyelid.

We split the parameters that need to be predicted into three subsets:
\begin{itemize}
    \item \emph{head pose} set $\boldsymbol{\theta_{p}^{'}}$, that contains both the rigid head pose $\boldsymbol{\theta_{p}}$ and the orthographic camera parameters~$\boldsymbol{c}$, forming a global representation of the head spatial placement. 
    \item \emph{identity} set $\boldsymbol{\beta}^{'}$, that only contains the typical identity shape parameters.
    \item \emph{expression} set $\boldsymbol{\psi}^{'}$, that contains the expression parameters $\boldsymbol{\psi}$ (extended with eyelid closure) along with jaw parameters $\boldsymbol{\theta}_{jaw}$. This set is responsible of controlling any possible facial expression. 
\end{itemize}
% \textcolor{red}{check this subsets - not to be confused with typical definitions in FLAME!}
After prediction, these parameters are used to differentiably render an image of the \textbf{geometry} of the 3DMM, denoted as $S$. Next, $S$ is concatenated along with a masked version $M(I)$ of the original input image, and the combined result is fed into an image-to-image generator which tries to reconstruct the original input image I (denoted as $I^{'}$).

%As it seems the overall concept of our method is simple: in order to minimize the reconstruction loss between the reconstructed image $I^{'}$ and the input image $I$, the image encoder $E$ is forced to capture facial shape and expression details, so that these can then be used to successfully guide the generator $D$ in his reconstruction.
 


Having described the functionality of the two core models, let us delve into the critical architectural details. 
%One common denominator for both models is the simplicity 

\qheading{Encoder}

As stated before, \emph{Encoder} estimates a set of FLAME parameters. In this work, we focus only on the expression part, training a network to jointly predict the 50 expression parameters, the 3 jaw pose parameters and the 2 eyelid parameters in order to fully control the facial expressions. 
Different networks are used for pose estimation and identity shaping so as to not interfere with the main expression predictor model. 
Overall, we used three distinct models to predict different sets of the FLAME parameters.
For all three models, we used MobileNetv3 architectures~\cite{}, aiming towards a lightweight backbone. 

\qheading{Image-to-Image Translator}

Given a rendered mesh of the 3D face and the masked-out input image, the \emph{Image-to-Image Translator} tries to reconstruct the initial image. This process is essentially an image-to-image translation (even though the initial ``image" is a concatenation of two images) and thus a UNet architecture~\cite{} is adopted. Its functionality relies on the usage of the estimated 3D geometry to reconstruct the initial faces characteristics.  
\textcolor{red}{Note that the non-textured rendered mesh is used as input. Preliminary experimentation showed no difference in performance when the texture from DECA was added.}    

A crucial property of this module is to assist the gradient flow towards the encoder. 
This way, both the reconstruction path and the cycle path will be more easily trained and ``collapsing" of solutions (e.g., generating non-realistic reconstructions) can be avoided. 
Therefore, a UNet-based architecture is ideal for this module, since the existing shortcut connection allow the gradient to flow uninterrupted. 

\textcolor{red}{check this}
The Image-to-Image Translator can be seen as a neural renderer alternative. 
However, contrary to such approaches, we do not aim to have a realistic rendering per-se, but rather have a lightweight and elegant guided \emph{inpainting} approach that heavily relies on the 3D geometry. 
This will be further highlighted by the masking step. 

%remove inner face 
%+ 
%add (very few) random pixels on the interior of the masked out face.
%Use them as guidance for reconstruction
\iffalse
\subsubsection{Pose Pre-training}

The proposed methodology assumes a stable face pose. In fact, preliminary experimentation, where pose was also optimized along the other FLAME parameters, shown sub-par performance, where expressions were mode ``plain". 
This can be attributed to the face position ``jittering", when pose is optimized, that complicates the visual reconstruction step. 
Thus, we consider a pre-trained pose estimation model that is ``frozen" during the training of our main framework. 
The pose could be taken from a different model (e.g., DECA).
In this work, we simply trained a pose estimation MobileNet only on landmarks information \textcolor{red}{@filby!!!}.
\fi

\subsubsection{Reconstruction Path}

The reconstruction path, as outlined in Figure~\ref{fig:reconstruction}, is the core pipeline for the proposed visual reconstruction scheme.
The process is straightforward: project the input image into the FLAME parameter space through the Encoder and use the rendered 3D face image along with a masked image to reconstruct the input image through the Image-to-Image Translator. 


\textbf{Rendering:}
\textcolor{red}{@filby}

visualize a part of FLAME rendering. mouth and eyes are ``empty".


\textbf{Impact of Masking:}

To promote the reliance from the 3D rendered face, we need to ``remove" the face of the input image. 
Specifically, we use the convex hull of detected 2D landmarks~\cite{bulat2017far} and dilate it in order to completely cover the input face.
The precision of the landmarks' position is not critical, since this masking out step aims to simply remove the inner structure of the face.

Without any information of face interior, training the Image-to-Image Translator becomes challenging. For example, texture information, such as skin color, facial hair or even accessories (e.g., glasses) are ``distractors" that complicate training. 
One way to address this issue, is to keep a small number of pixels from the interior of the face mask. 
Specifically, we retain a very small amount ($0.5\%$) of pixels, randomly selected, to be used as a guidance for reconstruction.
Note that if we use a larger number of pixels, the reconstruction becomes too guided, akin to an inpainting process, and the 3D rendered face does not control the reconstruction output adequately and the cycle path cannot faithfully reconstruct new expressions. 

A final addition to the masking process is done by extracting a mask of the rendered 3D face and allowing random pixels from the face interior that lie into this mask. 
The idea behind this extra step is to also mask-out pixels from inside the mouth and thus penalize ``heavy" inpainting actions, such as extending the lips because a pixel that correspond to lip was found inside the predicted mouth region. 
An example of such an erro can be seen in Figure~\ref{fig:masking_error}.
%This is very helpful for the cycle path also. 

%In the interior of the masked out face we retain a very small amount ($\approx 1\%$) of pixels which we have found out can be used as a guidance for reconstruction (?@george) and helps convergence.
%In order to mask the face during training we use the convex hull of detected 2D landmarks~\cite{bulat2017far} and dilate it in order to cover the input face. In the interior of the masked out face we retain a very small amount ($\approx 1\%$) of pixels which we have found out can be used as a guidance for reconstruction (?@george) and helps convergence.

As a sidenote, we initially experimented with randomly masking out a percentage of the input image, as done in~\cite{Autolink}, instead of placing the mask that covers the input face, however this did not provide satisfying results. 
Again, the main reason is that the model, in many cases, did not learn to fully utilize the 3D rendered face, but was oriented more towards inpainting the missing pixels. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/masking-procedure-cropped.pdf}
    \caption{+++.}
    \label{fig:masking_procedure}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/masking_error-cropped.pdf}
    \caption{Impact of rendered face mask on the overall masking scheme. If points are used from within the mouth, the system can learn an inpainting solution that resembles a closed mouth, even if this is not the case.}
    \label{fig:masking_error}
\end{figure}

\textbf{Considered Losses:}

\textcolor{red}{may add mathematical formulation of losses}

Optimization of such a reconstruction scheme, can be formulated through a loss that compares the reconstructed image with the initial one. 
To further enhance the performance of the proposed framework a set of losses is considered, as described below.
\begin{itemize}
    \item \emph{Image Reconstruction Losses:}
    %reconstruction loss: perceptual \& L1
%both losses required for the best possible results. (VGG-based) perceptual loss helps the fast convergence of a meaningful structure of the face, while L1 helps with appearance finer details.
    Reconstruction is optimized through two complementary losses. Specifically, we minimize the difference of the original image and the reconstructed image by 1) the perceptual loss of \cite{johnson2016perceptual} that uses multi-scale features and promotes structure similarity, as done in Autolink~\cite{}, and 2) $L_1$ loss. 
    The VGG-based perceptual loss helps the fast convergence of a meaningful structure of the face, while $L_1$ loss helps with the appearance of finer details.
    \item \emph{Landmark Loss:}
    Typical landmark loss is considered between detected landmarks of the input image and the corresponding landmarks, extracted from the 3D FLAME model. \textcolor{red}{@filby - more details}. \textcolor{red}{This loss acts as a guidance and has been proven not crucial for the proposed framework - remove it if no ablation is given}.
    \item \emph{Regularization:}
    We also use $L_2$ regularization over the expression parameters. This is complementary to the landmark loss in the sense of acting as a constraint to avoid extreme, non-realistic, expressions. 
    A shape regularizer is also in place to impose identity shaping with respect to a pre-trained network, such as DECA~\cite{feng2021learning} or MICA~\cite{zielonka2022mica}. 
    \item \emph{Task-Specific Perceptual Losses:}
    Finally, one can consider task-specific perceptual losses, that model adequately well subspaces of the expression space. Specifically, two such losses were considered: \emph{emotion loss}, as done in EMOCA~\cite{danecek2022emoca} and \emph{lip-read loss}, as done in SPECTRE~\cite{filntisis2023spectre}. Both losses employ pre-trained networks, trained specifically for the respective tasks, and used ``frozen" to back-propagate perceptual information to our models. In more detail, we also ``freeze" the Image-to-Image Translator for this step, and optimize only the Encoder, since we do not want these losses to affect the Image-to-Image Translator. 
    It should be noted that these losses lead to over-exaggeration of some expressions if not regularized properly; the simplest way to do this is by using the landmark loss with a non-trivial weight.
    The benefit of using such perceptual losses over the proposed framework is that the domain gap problem is minimized, since the two compared images are in the same space (e.g., EMOCA/SPECTRE used a texture-rendered image for comparison). 
    
\end{itemize}

%\textbf{Training of the Encoder:}


\subsubsection{Cycle Path}

%It's not only about consistency - it promotes (quite aggressively) variations

The aforementioned reconstruction concept could be a powerful tool but is constrained form the initial encoder parameters. 
For example, if a more complex lip structure cannot be reproduced quickly enough from the encoder, the generator learn to correlate miss-aligned lip structure and thus multiple different geometries of the lips will be collapsed to a single generator representation. 

This issue can be partially addressed with a cycle consistency path, where different FLAME parameters should be successfully retrieved through reconstructed images. 
The basic concept is straightforward: start from the FLAME parameter space, reconstruct a realistic image with the generator and then re-estimate the FLAME parameters using the encoder. 
This concept is visualized in Figure~\ref{fig:cycle}.
%We start from a set of FLAME parameters, we render the corresponding mesh and then we reconstruct a realistic face.  
Then a cycle consistency loss is directly used on the parameter space, enforcing the predicted FLAME parameters to be as close as possible to the initial ones.  
\textcolor{red}{refer to works with similar motivation and cycle losses}

\textbf{Promoting Diverse Expressions:}

Nonetheless, such a consistency loss alone is not enough to distinguish between the many possible facial expressions. If any of these paths, reconstruction or cycle, does not contains meshes with ``complex" structure the aforementioned expression collapse to a reduced set of reconstructed face images is unavoidable. 
To this end, this cycle path does not only enforce cycle consistency, but most importantly promotes variations in the expression parameter space.    
This way, we let the system ``see" expression parameters that typically are not that common.

To effectively augment the cycle path with interesting variations, the following steps are considered:
\begin{itemize}
%\item extend the batch be repeating K times
\item permute expressions in a batch
\item add noise on expression
\item use templates of ``difficult" / scarce expressions 
\item similar to the template case, enforce eyelids to close individually in this path
\end{itemize}

\textcolor{red}{add images to highlight augmentation}

\begin{figure*}
    \centering
    \includegraphics[width=.95\linewidth]{figures/cycle_expressions-cropped.pdf}
    \caption{++}
    \label{fig:cycle_expressions}
\end{figure*}

\textcolor{red}{Note that permuting expressions within a batch is a simple yet effective solution. However, to unlock the potential of such a solution, at least a subset of the training dataset should contain ``intense" expressions (e.g., emotion). Then the permutation step will transfer this expressions to the whole training set.} 


\textbf{Considered Losses:}

Here, the main loss is the mean-squared error between the initial expression parameters and the predicted at the end of the cycle path. 
The optimization is performed on both the Encoder and the Image-to-Image Translator, opting to fine-tune their functionality and impose consistency. 
Essentially, a one-to-one correspondence is desired between the 3D FLAME face and the reconstructed image. 

A potential problem with this extra cycle path is that the Image-to-Image Translator can be ``over-fitted" in order to create a non-realistic, render-like plain reconstruction \textcolor{red}{(see Figure~\ref{fig:cycle_error})}, since no supervision is in place to retain realistic images in this path. 
We have seen that with appropriate weight on the aforementioned cycle loss, we can avoid this problem, but the sensitivity remains.
This issue can be addressed by introducing an additional identity loss, that constraints the generated image to correspond to the same person as the initial input image. 
As the identity loss, the \textcolor{red}{@filby} is used. 

\textcolor{red}{may delete this} Moreover, we have evaluated the identity score on the considered datasets and we observed that images of the same person take values in the range $(0.1, 0.4)$, while different persons score above $0.5$. Therefore, we added a threshold to the optimization of the identity loss, set at $0.3$. Further optimizing the loss, below such a threshold, tries to make the images identical.


\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/cycle_error-cropped.pdf}
    \caption{\textcolor{red}{potential error of non-realistic reconstruction in the cycle path when no identity loss is used. - better for appendices}}
    \label{fig:cycle_error}
\end{figure}

\textbf{Face Image Manipulation}

A by-product of the proposed methodology is the creation of a well-performing face manipulation system, despite the simplicity of the translator.

\iffalse
%\subsection{Loss Formulation}

%reconstruction loss: perceptual \& L1
%both losses required for the best possible results. (VGG-based) perceptual loss helps the fast convergence of a meaningful structure of the face, while L1 helps with appearance finer details.

%cycle loss (MSE)

%(NOT NEEDED) landmark loss as guidance (minor impact)

\subsubsection{Extra perceptual losses}

Extra considered losses for ablation:
emotion, lip read.

Note that the considered domain is the reconstructed images, thus no domain gap exists. 

\fi


%\subsubsection{Face Image Manipulation}

%A by-product of the proposed methodology is the creation of a well-performing face manipulation system, despite the simplicity of the generator.

\subsubsection{Implementation Details?}

\todo{pretrain details?}







==> sections_camera_ready/tables/emotion_recognition/table.tex <==

% \begin{tabular}{l|cccc|cccc|c}
% \toprule
%         Model &  V-PCC $\uparrow$ &  V-CCC $\uparrow$ &  V-RMSE $\downarrow$ &  V-SAGR $\uparrow$ &  A-PCC $\uparrow$ &  A-CCC $\uparrow$ &  A-RMSE $\downarrow$ &  A-SAGR $\uparrow$ &  E-ACC $\uparrow$ \\
% \midrule
%         % ResNet 50     &  0.79 &  0.78 &   0.31 &   0.82 &  0.70 &  0.69 &   0.30 &   0.81 &     0.72 \\
%         % EmoNet Original     &  0.75 &  0.73 &   0.32 &   0.80 &  0.68 &  0.65 &   0.29 &   0.78 &     0.68 \\
%         MGCNet              &  0.71 &  0.69 &   0.35 &   0.80 &  0.59 &  0.58 &   0.34 &   0.77 &     0.60 \\
%         3DDFA-v2            &  0.63 &  0.62 &   0.39 &   0.75 &  0.53 &  0.50 &   0.34 &   0.73 &     0.52 \\
%         Deep3DFace          &  0.75 &  0.73 &   0.33 &   0.80 &  0.66 &  0.65 &   0.31 &   0.78 &     0.65 \\
%         DECA                &  0.70 &  0.69 &   0.36 &   0.76 &  0.59 &  0.58 &   0.33 &   0.74 &     0.59 \\
%         FOCUS-CelebA        &  0.70 &  0.69 &   0.35 &   0.78 &  0.57 &  0.54 &   0.33 &   0.75 &     0.58 \\
%         EMOCA v1            &  0.78 &  0.77 &   0.31 &   0.81 &  0.69 &  0.68 &   0.30 &   0.81 &     0.68 \\
%         EMOCA v2            &  0.77 &  0.76 &   0.33 &   0.81 &  0.67 &  0.66 &   0.30 &   0.76 &     0.66 \\ \hline
%         % Ours EMO 10       &  0.75 &  0.74 &   0.33 &   0.81 &  0.66 &  0.65 &   0.30 &   0.77 &     0.63 \\
%         % Ours EMO 5        &  0.73 &  0.71 &   0.34 &   0.80 &  0.66 &  0.65 &   0.30 &   0.78 &     0.64 \\
%         \modelName          &  0.74 &  0.73 &   0.34 &   0.79 &  0.66 &  0.65 &   0.31 &   0.77 &     0.64 \\
%         % Ours EMO 1        &  0.74 &  0.72 &   0.33 &   0.79 &  0.63 &  0.61 &   0.32 &   0.75 &     0.62 \\
%   \modelName w/o emo loss   &  0.73 &  0.72 &   0.34 &   0.80 &  0.62 &  0.61 &   0.32 &   0.75 &     0.62 \\
% \bottomrule
% \end{tabular}


\setlength\tabcolsep{1.5pt}
\begin{tabular}{l|cc|cc|c}
\toprule
        Model &  V-CCC $\uparrow$ &  V-RMSE $\downarrow$ &  A-CCC $\uparrow$ &  A-RMSE $\downarrow$ &  E-ACC $\uparrow$ \\
\midrule
        MGCNet              &  0.69 &   0.35 &  0.58 &   0.34 &     0.60 \\
        3DDFA-v2            &  0.62 &   0.39 &  0.50 &   0.34 &     0.52 \\
        Deep3DFace          &  0.73 &   0.33 &  0.65 &   0.31 &     0.65 \\
        DECA                &  0.69 &   0.36 &  0.58 &   0.33 &     0.59 \\
        FOCUS-CelebA        &  0.69 &   0.35 &  0.54 &   0.33 &     0.58 \\
        EMOCA v1            &  0.77 &   0.31 &  0.68 &   0.30 &     0.68 \\
        EMOCA v2            &  0.76 &   0.33 &  0.66 &   0.30 &     0.66 \\ \hline
        \modelName          &  0.73 &   0.34 &  0.65 &   0.31 &     0.64 \\
  \modelName w/o emo   &  0.72 &   0.34 &  0.61 &   0.32 &     0.62 \\
\bottomrule
\end{tabular}

==> sections_camera_ready/tables/emotion_recognition/table_exhaustive.tex <==

\begin{tabular}{l|cccc|cccc|c}
\toprule
                   Model &  V-PCC $\uparrow$ &  V-CCC $\uparrow$ &  V-RMSE $\downarrow$ &  V-SAGR $\uparrow$ &  A-PCC $\uparrow$ &  A-CCC $\uparrow$ &  A-RMSE $\downarrow$ &  A-SAGR $\uparrow$ &  E-ACC $\uparrow$ \\
\midrule
                                         ResNet 50     &  0.79 &  0.78 &   0.31 &   0.82 &  0.70 &  0.69 &   0.30 &   0.81 &     0.72 \\
                                   % EmoNet Original     &  0.75 &  0.73 &   0.32 &   0.80 &  0.68 &  0.65 &   0.29 &   0.78 &     0.68 \\
                                     MGCNet            &  0.71 &  0.69 &   0.35 &   0.80 &  0.59 &  0.58 &   0.34 &   0.77 &     0.60 \\
                                   3DDFA-v2            &  0.63 &  0.62 &   0.39 &   0.75 &  0.53 &  0.50 &   0.34 &   0.73 &     0.52 \\
                                 Deep3DFace            &  0.75 &  0.73 &   0.33 &   0.80 &  0.66 &  0.65 &   0.31 &   0.78 &     0.65 \\
                                              DECA     &  0.70 &  0.69 &   0.36 &   0.76 &  0.59 &  0.58 &   0.33 &   0.74 &     0.59 \\
                                      FOCUS-CelebA     &  0.70 &  0.69 &   0.35 &   0.78 &  0.57 &  0.54 &   0.33 &   0.75 &     0.58 \\
                                    EMOCA v1           &  0.78 &  0.77 &   0.31 &   0.81 &  0.69 &  0.68 &   0.30 &   0.81 &     0.68 \\
                             EMOCA v2                  &  0.77 &  0.76 &   0.33 &   0.81 &  0.67 &  0.66 &   0.30 &   0.76 &     0.66 \\ \hline
  %   Ours nolipread\_meadlrsceleb\_emotion1\_encoder\_9 &  0.73 &  0.72 &   0.34 &   0.80 &  0.62 &  0.61 &   0.32 &   0.78 &     0.62 \\
  %                       Ours from\_zero2\_4090swe\_38  &  0.72 &  0.71 &   0.35 &   0.78 &  0.60 &  0.59 &   0.33 &   0.73 &     0.61 \\
  % Ours wshape\_wpretrain2\_nolipread\_meadlrsceleb\_32 &  0.73 &  0.71 &   0.34 &   0.80 &  0.63 &  0.62 &   0.32 &   0.78 &     0.62 \\
  %         Ours wpretrain2\_nolipread\_meadlrsceleb\_9  &  0.71 &  0.71 &   0.36 &   0.78 &  0.59 &  0.58 &   0.33 &   0.73 &     0.61 \\
                                       % Ours EMO 10     &  0.75 &  0.74 &   0.33 &   0.81 &  0.66 &  0.65 &   0.30 &   0.77 &     0.63 \\
                                       %  Ours EMO 5     &  0.73 &  0.71 &   0.34 &   0.80 &  0.66 &  0.65 &   0.30 &   0.78 &     0.64 \\
                                        Ours EMO 2 &  0.74 &  0.73 &   0.34 &   0.79 &  0.66 &  0.65 &   0.31 &   0.77 &     0.64 \\
                                        % Ours EMO 1     &  0.74 &  0.72 &   0.33 &   0.79 &  0.63 &  0.61 &   0.32 &   0.75 &     0.62 \\
                                        % Ours EMO 0     &  0.73 &  0.72 &   0.34 &   0.80 &  0.62 &  0.61 &   0.32 &   0.75 &     0.62 \\
\bottomrule
\end{tabular}

